Robust Real-time Computing with Chemical Reaction Networks

Recent research into analog computing has introduced new notions of computing real numbers. Huang, Klinge, Lathrop, Li, and Lutz defined a notion of computing real numbers in real-time with chemical reaction networks (CRNs), introducing the classes $\mathbb{R}_\text{LCRN}$ (the class of all Lyapunov CRN-computable real numbers) and $\mathbb{R}_\text{RTCRN}$ (the class of all real-time CRN-computable numbers). In their paper, they show the inclusion of the real algebraic numbers $ALG \subseteq \mathbb{R}_\text{LCRN} \subseteq \mathbb{R}_\text{RTCRN}$ and that $ALG \subsetneqq \mathbb{R}_\text{RTCRN}$ but leave open where the inclusion is proper. In this paper, we resolve this open problem and show $ALG= \mathbb{R}_\text{LCRN} \subsetneqq \mathbb{R}_\text{RTCRN}$. However, their definition of real-time computation is fragile in the sense that it is sensitive to perturbations in initial conditions. To resolve this flaw, we further require a CRN to withstand these perturbations. In doing so, we arrive at a discrete model of memory. This approach has several benefits. First, a bounded CRN may compute values approximately in finite time. Second, a CRN can tolerate small perturbations of its species' concentrations. Third, taking a measurement of a CRN's state only requires precision proportional to the exactness of these approximations. Lastly, if a CRN requires only finite memory, this model and Turing machines are equivalent under real-time simulations.

==> body/macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumitem}
\usepackage{ifthen}
\usepackage{mathrsfs}
\usepackage{mathabx}
\usepackage{mathtools}
\usepackage[textsize=scriptsize]{todonotes}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{xspace}
\usepackage[margin=1in]{geometry}

\RequirePackage[final]{microtype}
\DisableLigatures{encoding = T1, family = tt* }

\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\eg}{e.g.\@\xspace}

\makeatletter
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\makeatother

\makeatletter
\newcommand*{\etal}{%
    \@ifnextchar{.}%
        {et al}%
        {et al.\@\xspace}%
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem Commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{observation}[theorem]{Observation}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
	
\newcommand{\qed}{\begin{flushright} \setlength{\parskip}{-1em} $\square$ \end{flushright}}

\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\set}{\{}{\}}
\DeclarePairedDelimiter{\abs}{|}{|}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\inner}{\langle}{\rangle}
\DeclarePairedDelimiter{\interval}{[}{]}

\newcommand{\collection}[4][]
{
	\ifthenelse{\equal{#1}{}}
	{\set*{#2}_{#3 \in #4}}
	%else
	{\set*{#1}_{#2 = #3}^{#4}}
}

\newcommand{\func}[3][]
{
	\ifthenelse{\equal{#1}{}}
	{#2 \rightarrow #3}
	%else
	{#1 : #2 \rightarrow #3}
}

\newcommand{\iu}{{i\mkern1mu}}
\newcommand{\conj}{\overline}
\newcommand{\magn}[1]{\abs*{#1}}

\newcommand{\tuple}[1]{\paren*{#1}}
\newcommand{\card}[1]{\abs*{#1}}

\newcommand{\powerset}[1]{\mathscr{P} \paren*{#1}}

\newcommand*{\union}{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}}
\newcommand*{\intersect}{\mathbin{\scalebox{1.5}{\ensuremath{\cap}}}}

\newcommand{\naturals}{\mathbb{N}}
\newcommand{\extendednaturals}{\overline{\mathbb{N}}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\bin}{\mathbb{Z}_{2}}
\newcommand{\pints}{\mathbb{Z}^{+}}
\newcommand{\nints}{\mathbb{Z}^{-}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\extendedreals}{\overline{\reals}}
\newcommand{\nnr}{\reals_{\ge 0}}
\newcommand{\positives}{\reals^{+}}
\newcommand{\negatives}{\reals^{-}}
\newcommand{\alg}{ALG}
\newcommand{\lcrn}{\mathbb{R}_\text{LCRN}}
\newcommand{\rtcrn}{\mathbb{R}_\text{RTCRN}}
\newcommand{\comp}{\mathbb{R}_\text{COMP}}

\newcommand{\iso}{\approx}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\Mod}[1]{\ \text{mod}\ #1}
\newcommand{\ord}[1]{\abs*{#1}}

\newcommand{\odx}[2]{\frac{d #1}{d #2}}
\newcommand{\pdx}[2]{\frac{\partial #1}{\partial #2}}

\newcommand{\lsq}[1]{\ell^2(#1)}
\newcommand{\pnorm}[2]{\norm*{#1}_{#2}}

\newcommand{\pmf}[2]{\func{#1}{#2}{\interval*{0,1}}}
\newcommand{\pmfnz}[2]{\func{#1}{#2}{\left( 0,1 \right]}}
\newcommand{\cov}[3][]
{
	\ifthenelse{\equal{#1}{}}
	{cov \paren*{#2,#3}}
	{cov_{#1} \paren*{#2,#3}}
}

\newcommand{\meas}[2]{\func{#1}{\pow{#2}}{\mathbb{R}_{\ge 0}}}

\newcommand{\tageq}[1]{\tag{\arabic{equation}} \label{#1} \stepcounter{equation}}
